Dynamic Computational Time for Visual Attention

We propose a dynamic computational time model to accelerate the average processing time for recurrent visual attention (RAM). Rather than attention with a fixed number of steps for each input image, the model learns to decide when to stop on the fly. To achieve this, we add an additional continue/stop action per time step to RAM and use reinforcement learning to learn both the optimal attention policy and stopping policy. The modification is simple but could dramatically save the average computational time while keeping the same recognition performance as RAM. Experimental results on CUB-200-2011 and Stanford Cars dataset demonstrate the dynamic computational model can work effectively for fine-grained image recognition.The source code of this paper can be obtained from https://github.com/baidu-research/DT-RAM

==> Makefile <==
# TARGET=egpaper_for_review
TARGET=egpaper_final

all: 
	pdflatex $(TARGET).tex
	#detex $(TARGET).tex | grep -v '^$$' > $(TARGET).txt
	bibtex $(TARGET)
	pdflatex $(TARGET).tex
	pdflatex $(TARGET).tex
	rm -f $(TARGET).synctex $(TARGET).aux $(TARGET).log $(TARGET).bbl $(TARGET).blg $(TARGET).brf $(TARGET).txt $(TARGET).out

clean:
	rm -f $(TARGET).synctex $(TARGET).aux $(TARGET).log $(TARGET).bbl $(TARGET).blg $(TARGET).brf $(TARGET).txt $(TARGET).out
	rm -f *.log
	find . -name '*.eps' -exec rm -v {} \; 

show: all
	evince $(TARGET).pdf

